New Streaming Algorithms for High Dimensional EMD and MST

We study streaming algorithms for two fundamental geometric problems: computing the cost of a Minimum Spanning Tree (MST) of an $n$-point set $X \subset \{1,2,\dots,\Delta\}^d$, and computing the Earth Mover Distance (EMD) between two multi-sets $A,B \subset \{1,2,\dots,\Delta\}^d$ of size $n$. We consider the turnstile model, where points can be added and removed. We give a one-pass streaming algorithm for MST and a two-pass streaming algorithm for EMD, both achieving an approximation factor of $\tilde{O}(\log n)$ and using polylog$(n,d,\Delta)$-space only. Furthermore, our algorithm for EMD can be compressed to a single pass with a small additive error. Previously, the best known sublinear-space streaming algorithms for either problem achieved an approximation of $O(\min\{ \log n , \log (\Delta d)\} \log n)$ [Andoni-Indyk-Krauthgamer '08, Backurs-Dong-Indyk-Razenshteyn-Wagner '20]. For MST, we also prove that any constant space streaming algorithm can only achieve an approximation of $\Omega(\log n)$, analogous to the $\Omega(\log n)$ lower bound for EMD of [Andoni-Indyk-Krauthgamer '08]. Our algorithms are based on an improved analysis of a recursive space partitioning method known generically as the Quadtree. Specifically, we show that the Quadtree achieves an $\tilde{O}(\log n)$ approximation for both EMD and MST, improving on the $O(\min\{ \log n , \log (\Delta d)\} \log n)$ approximation of [Andoni-Indyk-Krauthgamer '08, Backurs-Dong-Indyk-Razenshteyn-Wagner '20].

==> Sketching.tex <==
%!TEX root = MST.tex


\subsection{Useful Facts}

We begin with some useful facts. We first define stable random variables.
\begin{definition}\label{def:stable}
	A distribution $\mathcal{D}$ is said to be $p$-stable if whenever $X_1,\dots,X_n \sim \mathcal{D}$ are drawn independently and $a \in \R^n$ is a fixed vector, we have
	\[	\sum_{i=1}^n a_i X_i = \|a\|_p X	\]
	where $X \sim \mathcal{D}$ is again drawn from the same distribution, and the ``$=$'' symbol above denotes distributional equality. For $p \in (0,2]$, we define the \textit{standard $p$-stable distribution}, denoted $\cD_p$, to be the distribution with characteristic function 
	\[\exx{Z \sim \cD_p}{e^{itZ}	} = e^{-|t|^p}\]
	which is, in fact, is $p$-stable. %In particular, for $p=2$, the standard $2$-stable distribution $\cD_2$ is just the normal distribution $\mathcal{N}(0,1)$ (i.e., $\sum_i a_i g_i = g \cdot \|a\|_2$, where $g,g_1,\dots,g_n$ are Gaussian), and the standard $1$-stable distribution $\cD_1$ is the \textit{Cauchy Distribution}.
\end{definition}
Standard methods for generating $p$-stable random variables are discussed in \cite{nolan2009stable}.
%Note for $p<2$, the distributions have heavy tails -- namely we have the following fact.
%\begin{fact}[Chapter 1.5 \cite{nolan2009stable}]\label{fact:pstabletail}
%	Fix $p \in (0,2)$, and let $\cD_p$ be the standard $p$-stable distribution. Then there is a constant $C_p$ depending only on $p$, such that for any $t >0$, we have
%	\[	\lim_{t \to \infty } \frac{\prb{X \sim \cD_p}{|X| > t}}{C_p \frac{1}{t^p}}= 1	\]
%\end{fact}



\begin{proposition}[\cite{chambers1976method}]\label{prop:genstable}
	Fix any $p \in (0,1)$. Then $X \sim \cD_p$ can be generated as follows:
	\begin{enumerate}
		\item Generate $\theta \sim \text{Uniform}[-\frac{\pi}{2},\frac{\pi}{2}]$.
		\item Generate $r \sim \text{Uniform}[0,1]$.
		\item Set 
		\[X \leftarrow \frac{\sin(p \theta)}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\]
	\end{enumerate}
	\end{proposition}

By Proposition \ref{prop:genstable}, it follows that if we want to generate $X \sim |\cD_p|$, we can generate $\theta \sim \text{Uniform}[-\frac{\pi}{2},\frac{\pi}{2}]$ and $r \sim \text{Uniform}[0,1]$, and set 

\begin{align*}
X &= \left|  \frac{\sin(p \theta)}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\right| \\
&= \frac{|\sin(p \theta)|}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\\
\end{align*}
Notice that since $\cos(\theta(1-p))$ is symmetric around the origin in $\theta$, the entire function above is symmetric around the origin in $\theta$. Thus, we have the following corollary.

\begin{corollary}\label{cor:genstable}
	Fix any $p \in (0,1)$. Then $X \sim |\cD_p|$ can be generated as follows:
	\begin{enumerate}
		\item Generate $\theta \sim \text{Uniform}[0,\frac{\pi}{2}]$.
		\item Generate $r \sim \text{Uniform}[0,1]$.
		\item Set 
		\[X \leftarrow \frac{\sin(p \theta)}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\]
	\end{enumerate}
\end{corollary}


In what follows, we define a function function $g(r,\theta): (0,1) \times (0,\pi/2) \to \R$ via
\[g(r,\theta) = \frac{\sin(p \theta)}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\]

We now prove some facts about $g(r,\theta)$

\begin{proposition}\label{prop:monotoneg}
	Define the function $g(r,\theta)$ as above, with the domain $(0,1) \times (0,\frac{\pi}{2})$. Then $g$ is monotone increasing in both parameters.
	\end{proposition}
\begin{proof}
First, fix any $\theta \in (0,\pi/2)$. Then since $\ln(1/r)$ is decreasing as $r$ increases in $(0,1)$ the value $(\frac{1}{\ln(1/r)})^{(1-p)/p}$ is monotone decreasing in $r$, as needed. For the second part, notice that $\sin(p \theta)$ is monotone increasing in $\theta$. Thus, it suffices to show that the function

\[	\frac{\cos(\theta(1-p))^{1-p}}{\cos(\theta)}	\]
is monotone increasing.  We have

\[\frac{\partial}{\partial \theta} \frac{\cos ^{1-p}(\theta (1-p))}{\cos (\theta )}=\tan (\theta ) \sec (\theta ) \cos ^{1-p}(\theta (1-p))\]

Note that all three of $\tan (\theta ), \sec (\theta ) ,$ and $\cos(\theta(1-p))$ are positive for $\theta \in (0,\pi/2)$, which completes the claim and the proof of the Proposition
\end{proof}

We obtain the following corollary.

\begin{corollary}
	Define the function $g(r,\theta)$ as above, with the domain $(0,1) \times (0,\frac{\pi}{2})$. Then we have
	\[|\median(\cD_p)| = g\left(\frac{1}{2},\frac{\pi}{4}\right)	\]
	Where $|\median(\cD_p)|$ is the value such that
	\[			\prb{X \sim \cD_p}{|X| < |\median(\cD_p)|} =1/2	\]
	\end{corollary}


\begin{lemma}\label{lemma:stablemedianbound}
	Fix any $p \in (0,1)$ and $\eps >0$, and let $R =|\median(\cD_p)|$.  Then there exists a constant $C$ independent of $p,\eps$ such that
	
	\[	\prb{X \sim \cD_p}{R \leq |X| \leq (1+  \eps)R} \geq C p^2 \eps^2  \]
	and 
		\[	\prb{X \sim \cD_p}{(1-\eps)R \leq |X| \leq R} \geq C p^2 \eps^2  \]
\end{lemma}
\begin{proof}
	Define the function $g(r,\theta)$ as above, and recall by Corollary \ref{cor:genstable} that we can generate $X \sim |\cD_p|$ by picking $r \sim [0,1],\theta \sim [0,\pi/2]$ and setting $X = g(r,\theta)$. Moreover, we know by the prior discussion that $R = g(1/2,\pi/4)$. We will proceed by bounding the partial derivatives of $\ln(g(r,\theta))$ by a value $\Omega(1/p)$ for any $r,\theta$ bounded away from the edges of the domain box $(0,1) \times (0,\pi/2)$. We have
	
	
	\[\frac{\partial}{\partial \theta}	\ln(g(r,\theta))  = \frac{\cos(p \theta)}{\sin (p \theta)} - \frac{(1-p)^2}{p} \frac{\sin(\theta(1-p))}{\cos(\theta(1-p))} + \frac{1}{p} \frac{\sin(\theta)}{\cos(\theta)}	\]
	
	For $\theta$ in the interval $(1/100,\pi/2 - 1/100)$, the above derivative is bounded in magnitude by $C_1 p^{-1}$, for some constant $C_1$. For the second partial derivative, we have
		\[\frac{\partial}{\partial r}	\ln(g(r,\theta)) =\frac{\partial}{\partial r} -(1-p)/p \ln(\ln(1/r))= \frac{1-p}{p}  \frac{1}{r \log(1/r)}  \]
	Again, for $r$ in the interval $[1/100,99/100]$, the above is bounded by $C_1 p^{-1}$. It follows that if $I_1 \times I_2$ is the product of any two intervals inside with $I_1 \subset (\frac{1}{100},\frac{99}{100}) $ and $I_2 \subset  (1/100,\pi/2-1/100)$ Then we have
	
	\[	\max_{(r_1,\theta_1),(r_2,\theta_2) \in I_1 \times I_2} \left|\ln(g(r_1,\theta_1)) - \ln(g(r_2,\theta_2)) \right| \leq \frac{C_1( |I_1| + |I_2|)}{p}	\]
	
It follows that for intervals $I_1,I_2$ with $|I_1| - |I_2| < c \eps  p $ for a sufficiently small constant $c$, it follows that 
	
		\[	\max_{(r_1,\theta_1),(r_2,\theta_2) \in I_1 \times I_2} \left|\frac{g(r_1,\theta_1)}{ g(r_2,\theta_2)} \right| \leq \exp\left(\frac{C_1( |I_1| + |I_2|)}{p} \right) \leq 1+ \eps	\]
	We apply the above fact with $I_1 = [1/2 - \gamma, 1/2 + \gamma]$ and $I_2 = (\pi/4 - \gamma, \pi/4 + \gamma)$, where $\gamma = c p \eps /4$. Let $I_1^+ = [1/2,1/2+ \gamma], I_1^- = [1/2 - \gamma, 1/2]$ and $I_2^+ =[\pi/4 , \pi/4 + \gamma$ and $I_2^- = [\pi/4 - \gamma, \pi/4]$. By the monotonicty of $g$ (Proposition \ref{prop:monotoneg}), and the above paragraphs, it follows that 
	$$R \leq g(r,\theta) \leq (1+\eps)R$$
	For all $(r,\theta) \in I_1^+ \times I_2^+$, and moreover 
	$$(1-\eps)R \leq g(r,\theta) \leq R$$
	For all $(r,\theta) \in I_1^- \times I_2^-$.
	Moreover, the area of both $I_1^+ \times I_2^+$ and $I_1^- \times I_2^-$ is $\Omega(p^2 \eps^2)$, from which it follows that the probability that $(r,\theta)$ is in $I_1^+ \times I_2^+$ is at least $\Omega(p^2 \eps^2)$, and similarly for $I_1^- \times I_2^-$, which completes the proof of the Lemma.

 


\end{proof}


We are now ready to prove the correctness of the Indyk $p$-stable sketch. 
\begin{theorem}[Indyk's $p$-Stable Sketch]\label{thm:indykPrelims}
Fix $1/2 > p > 0$ and $\eps \in (0,1)$, and set $t = \Theta(\frac{1}{(p\eps)^4} \log\delta^{-1})$ Let $\bX_1,\dots,\bX_t \sim \cD_p$ independently. Then, with probability $1-\delta$, we have
\[1-\eps\leq	\median_{i \in [t]} \left\{	\frac{|\bX_i|}{|\median(\cD_p)|}	\right\}  \leq 1+\eps		\]
Where $|\median(\cD_p)|$ is the value such that
\[			\prb{X \sim \cD_p}{|X| < |\median(\cD_p)|} =1/2	\]
\end{theorem}
\begin{proof}
	Set $R = |\median(\cD_p)|$. By Lemma \ref{lemma:stablemedianbound}, we have both $	\prb{X \sim \cD_p}{r \leq |X| \leq (1+\eps)r} = \Omega(p^2 \eps^2)$, and $\prb{X \sim \cD_p}{(1-\eps)r \leq |X| \leq r} = \Omega(p^2\eps^2)$. It follows that  there exists a constant $c>0$ such that for each trial $\bX_i$, the probability that $\bX_i > (1+\eps )R$ is at most $1/2 - c p^2 \eps^2$, and the probability that $\bX_i < (1-\eps)R$ is at most $1/2 - c p^2 \eps^2$.	
	 By Chernoff bounds, we have
	
	\[	\pr{ \left|	\left\{ i \in [t] \; | \; \bX_i > (1+\eps)R	\right\}	\right| \geq 1/2} < e^{- \eps^4 p^4  t/3} 	\]
	and 
			\[	\pr{ \left|	\left\{ i \in [t] \; | \; \bX_i < (1-\eps)R	\right\}	\right| \geq 1/2} < e^{- \eps^4 p^4  t/3} 	\]
	Conditioned on both of these events occurring simultaneously, which occurs with probability at least $1- 2 e^{- \eps^4 p^4  t/3} > 1-\delta$, the median must fall within the range $(1-\eps)R$ and $(1+\eps)R$. Thus, we have:
			\[	\pr{	\median_{i \in [t]} \left\{	\frac{|\bX_i|}{|\median(\cD_p)|} \right\}= (1\pm\eps) r} > 1-\delta	\]
		as needed.
			

\end{proof}

==> two-pass.tex <==

%!TEX root = main.tex

\section{Two-Round Linear Sketch}\label{sec:communication}

In this section and the following, we %demonstrate how 
leverage our improved analysis to design linear sketches for EMD over $\{0,1\}^d$; the extension to EMD over $(\R^d, \|\cdot\|_p)$ for $p \in [1,2]$ follows from a standard application of metric embeddings (see Appendix~\ref{app:ell_p}). %for EMD can be obtained in a \textit{sketching} algorithm. 
Specifically, we first demonstrate how a $\tilde{O}(\log s)$ approximation can be obtained using $\polylog( s, d)$ bits of space in %the
a \textit{two-round} linear sketching model (we give a formal description shortly). In the subsequent section, we implement the linear sketch in a single round, at the cost of a small additive error. In cases where sets $A, B$ do not substantially overlap, the one-round protocol %in most cases, will also 
yields the same multiplicative guarantee. As is relatively standard in the sketching literature, the two-round and one-round linear sketch may be used for two-round and one-round communication settings, as well as two-pass and one-pass streaming algorithms (see Appendix~\ref{app:formal-models} for a more thorough explanation of the model).

%We remark that the two-round and one-round communication settings correspond to the two-pass and one-pass, respectively, models of \textit{streaming}. Thus, we will see that our algorithms easily extend to one and two-pass streaming algorithms with the same space. We begin by formalizing this communication model, and its relation to streaming. Lastly, we will introduce the concept of \textit{linear-sketching} and two-round linear sketching. We will see that a linear sketch yields both a streaming and a communication algorithm, and is therefore the strongest of the three models. 
%For the following sections, we will work over the hypercube $\{0,1\}^d$ and the $\ell_1$ norm, with the understanding that our algorithms naturally extend to $\R^d$ and $\ell_p$ norms by the same embeddings as seen earlier, which can be computed in small space in a stream. For clarity, we will restrict the following discussion to communication, streaming, and sketching specifically in the context of estimating earth-mover's distance. 


\paragraph{Linear Sketching for EMD over $\{0,1\}^d$.} For some $m \in \N$, we encode the inputs of a computational problem as a vector $f$ in $\R^m$. For that encoding and a parameter $k \in \N$, a \emph{linear sketch} is a distribution over $k \times m$ matrices $\bS$, where ideally $k \ll m$, accompanied by an algorithm $\Alg_{\bS}$, which receives an input $\bS f \in \R^k$ and outputs an answer to the computational problem. The algorithm maintains the vector $\bS x$ in $k$ words of space and utilizes $\Alg_{\bS}$ to produce an output. In the public coin model, storing the random matrix $\S$ is not counted against the space complexity of the algorithm ($\S$ can often be stored in small space, such as for streaming, see Corollary \ref{cor:twopass}).
%Ideally $k \ll m$ and the matrix $\bS$ can be stored implicitly, in which case the algorithm maintains the vector $\bS x$ in $k$ words of space and utilizes $\Alg_{\bS}$ to produce an output. 
In order to define linear sketching for EMD over size-$s$ subsets of $\{0,1\}^d$, we must specify the encoding in $\R^m$, as well as the space complexity $k$, and the distribution over $k \times m$ matrices $\bS$ and decoding algorithms.

A pair of multi-sets $A, B \subset \{0,1\}^d$ is encoded as a vector $f_{A, B} \in \R^{2 \cdot 2^d}$, where the first $2^d$ coordinates represent the indicator vector of $A$ in $\{0,1\}^d$, and the second $2^d$ coordinates represent the indicator vector of $B$ in $\{0,1\}^d$. More precisely, for $i \in \{0,1\}^d$, the $i$-th coordinate (in standard binary encoding) of $f_{A, B}$ is the number of points in $A$ at $i$; the $(2^d + i)$-th coordinate of $f_{A,B}$ is the number of points in $B$ at $i$.

The two-round linear sketch is defined by a linear sketch which produces an intermediate output for the first round, and another linear sketch (parametrized by the output of the first round) which produces the final output. Specifically, we have distribution $\calD^{(1)}$ supported on $k \times 2 \cdot 2^d$ matrices, as well a decoding algorithm for a vector $\by_1 = \bS_1 f_{A,B} \in \R^k$. In one-round sketching, the output is produced by the decoding algorithm. For two-round round linear sketching, we consider another distribution $\calD^{(2)}$, parametrized by the decoding of $\by_1$, as well as $\bS_1$, supported on $k \times 2 \cdot 2^d$ matrices $\bS_2$, as well as a decoding algorithm for a vector $\by_2 = \bS_2 f_{A,B} \in \R^k$ which produces the output.

\subsection{The Two-Round Linear Sketching Algorithm}



In this section, we give a two-round linear sketching algorithm for approximating the Earth Movers distance. Recall that 
for a linear sketch, the multisets $A,B \subset \{0,1\}^d$ are \textit{implicitly} encoded as a vector $f_{A,B} \in \R^{2^{d+1}}$ which indicates the members and frequencies of the points in $A,B$. %Recall further that a two round sketching protocol generates a random matrix $\S_1$, and based on knowledge only of $\S_1,\S_1 f_{A,B}$, the algorithm adaptively generates another random matrix $S_2$. The final output is then a function only of $\S_1,\S_2,\S_1 f_{A,B}, \S_2 f_{A,B}$.
Specifically, we prove the following theorem.
 
 \begin{theorem}\label{thm:two-pass}
 	For $d,s \in \N$, there exists a 2-round linear sketching algorithm such that given multi-sets $A,B \subset \{0,1\}^d$ with $|A| = |B| = s$, computes an approximation $\hat{\calbI}$ to $\EMD(A,B)$ with
 	\[	\EMD(A,B) \leq \hat{\calbI} \leq \tilde{O}(\log s) \EMD(A,B) 	\]
 	with probability at least $3/4$. Moreover, the space of the linear sketch is $\polylog(s, d)$ bits.
 \end{theorem}
 
 
%\begin{theorem}\label{thm:two-pass}
%For $d,s \in \N$, there exists a 2-round communication protocol $\bPi$ using $\polylog(s, d)$ bits of communication which satisfies the following property: 
%\begin{itemize} 
%\item Alice receives a multi-set $A \subset \{0,1\}^d$ of size $s$, and 
%\item Bob receives a multi-set $B \subset \{0,1\}^d$ of size $s$, 
%\item The protocol $\bPi(A, B)$ outputs an estimate $\hat{\mathcal{I}} \in \R^{\geq 0}$ satisfying
%\begin{align*}
%\EMD(A, B) \leq \hat{\mathcal{I}} \leq \tilde{O}(\log s) \EMD(A, B)
%\end{align*}
%with probability at least $3/4$ over the randomness of the protocol.
%\end{itemize}
%\end{theorem}

%\begin{remark}
%{\color{red} Here, we should explain how the above protocol is a linear sketch -- however, we need to be careful in describing the alphabet of the stream.}
%\end{remark}

The protocol will proceed by sampling a compressed quadtree $\bT$ of depth $h = \log_2(2d)$, and for each depth $i \in \{ 0, \dots, h-1\}$, using $\ell_1$-sampling and $\ell_1$-sketching to estimate 
\begin{align*}
\cbI _i\eqdef \sum_{v \in \cV_i} \big| |A_v| - |B_v| \big| \cdot \bq_{\pi(v), v},
\end{align*}
up to a constant factor. We recall that for a node $v$ in the tree, the multi-sets
\begin{align*}
A_v &= \left\{ a \in A : \bv_{i}(a) = v\right\} \qquad\text{and}\qquad B_v = \left\{ b \in B : \bv_i(b) = v \right\} 
\end{align*}
are the points from $A$ and $B$ which are mapped to node $v$ in the compressed quadtree $\bT$. The point 
\begin{align*}
\bc_v &= \frac{1}{|A_v \cup B_v|} \sum_{ x \in A_v \cup B_v} x,
\end{align*}
is the center of mass among all points which map to node $v$. We have that
\begin{equation}\label{eqn:bq}
\begin{split}
\bq_{u, v} &= \left\{ \begin{array}{cl} \frac{d}{2^i} &\|\bc_u - \bc_v\|_1 \leq \frac{d}{2^i} \vspace{0.2cm} \\
							\frac{30d\log s}{2^i} & \|\bc_u - \bc_v\|_{1} \geq \frac{30d\log s}{2^i} \vspace{0.2cm} \\
							\|\bc_u - \bc_v\|_1 & \text{ o.w.}  \end{array} \right. .
\end{split}
\end{equation}

Recall that by Remark~\ref{rem:sketching-value}, 
\[ \EMD(A, B) \leq \sum_{i=0}^{h-1} \calbI_i \leq \tilde{O}(\log s) \cdot \EMD(A, B), \]
with probability at least $0.89$ over the draw of $\bT$. Hence, the protocol produces an estimate $\hat{\calbI}_i \in \R$ where $\calI_i \leq \hat{\calbI}_i \leq O(1) \cdot \mathcal{I}_i$ with probability at least $1 - 1/(100h)$. Via a union bound over all $h$ levels of the tree as well as the good draw of $\bT$, we have that with probability at least $0.88$, $\sum_{i=0}^{h-1} \hat{\calbI}_i$ satisfies the requirements of Theorem~\ref{thm:two-pass}. See Figure~\ref{fig:2-round} for a description of the protocol which estimates $\calbI_i$ up to constant factor with high (constant) probability.


\subsubsection{Universe Reduction} Observe that $\cbI_i$ is a sum over $|\cV_i| = 2^{2^i}$ vertices of $\bT$. However, since $|A| = |B| = s$, at most $2s$ of these summands will be non-zero. Thus, we perform a standard universe reduction on the layer $(\cV_{i-1},\cV_{i})$ as follows. Select two fully independent hash functions $\bh_{i-1}:[\cV_{i-1}] \to [s'] ,\bh_{i}:[\cV_{i}] \to [s'] $, where $s' = O(s^3)$. We then define 
\[ \cV_{i-1}' = [s'], \qquad \text{and}\qquad \cV_i' = [s']\times [s'], \]
 and construct the bipartite graph $(\cV_{i-1}',\cV_{i}')$  corresponding to layers $i-1$ and $i$ of $\bT$ after a universe reduction. The nodes of $\cV_{i-1}'$ represent groups of nodes in $\cV_{i-1}'$ under the mapping $\bh_{i-1}$. The nodes of $\cV_{i}'$ are indexed by pairs $(y,z) \in [s']\times [s']$, where the index $y$ specifies the group of the parent node (under $\bh_{i-1}$), and $z$ represents group of child nodes in $\cV_i$. The edges are added to preserve parent-child relationships in $\cV_{i-1}'$ and $\cV_i'$: $(x,(y,z)) \in \cV_{i-1}' \times \cV_{i}'$ is added as an edge if $x=y$ for $x,y,z \in [s']$. (See Figure~\ref{fig:universe}.)

\begin{figure}
\centering
\begin{picture}(400, 100)
\put(40,0){\includegraphics[width=0.7\linewidth]{universe-reduction.pdf}}
\put(0, 103){$\calV_{i-1}:$}
\put(0, 73){$\calV_i:$}
\put(0, 37){$\calV_{i-1}':$}
\put(0,7){$\calV_i':$}
\end{picture}
\caption{An example of the universe reduction from the bipartite graph defined on $(\calV_{i-1}, \calV_i)$ to the bipartite graph defined on $(\calV_{i-1}', \calV_i')$, as well as the corresponding mapping from $\bh_{i-1}$ and $\bh_i$. The shaded regions correspond to pre-images of the node mappings.}
\label{fig:universe}
\end{figure}

For $x \in \cV_{i-1}' $ and  $(y,z)\in \cV_{i}' $, we can naturally define
\[A_x = \{a \in A: \bh_{i-1}(\bv_{i-1}(a)) = x	\} \quad A_{(y,z)} = \{a \in A: \bh_{i}(\bv_{i}(a)) = z, \bh_{i-1}(\bv_{i-1}(a)) = y\}\]
 We similarly define $B_u,B_v$ for $u \in \cV_{i-1}', v \in \cV_{i}'$. We can also define centers $\bc_v',\bc_u'$ of the sets $A_u\cup B_u,A_v\cup B_v$ where $u \in \cV_{i-1}',v\in \cV_i'$, and define  $\bq_{\pi(v), v}'$ identically to $\bq_{\pi(v), v}'$  but using the centers $\bc_{v}'$. Altogether, we can set
\[		\cbI_i' \eqdef \sum_{v \in \cV_i'} \big| |A_v| - |B_v| \big| \cdot \bq_{\pi(v), v}' \]
where $\pi(v) \in \cV_{i-1}'$ is the parent of $v$ in the new tree.
Notice that since both $\cV_i,\cV_{i-1}$ have at most $2s$ non-empty nodes each, with probability $1-1/s$ we have that $\bh_{i-1}$ and $\bh_{i}$ are injective into $[s']$ and $[s']^2$ respectively on the non-empty nodes (i.e., the non-empty nodes perfectly hash). Since $\cbI_i$ is just a sum over edges, if the non-empty edges perfectly hash, the construction of $\cbI_i'$ just amounts to a renaming of the non-zero edges. %Moreover, notice that the values $|A_v|, |B_v|, \bc_v$ are all still linear functions of $f_{A,B}$

\begin{proposition}\label{prop:unireduce}
	With probability $1-1/s$ over the choice of $\bh_{i-1},\bh_i$, we have $\cbI_i = \cbI_i'$. Moreover, the hash functions $\bh_{i-1},\bh_i$ need only be $2$-wise independent. %Moreover, this occurs conditioned on an event $\calbE_0$ that $h_{i}(u) \neq h(u')$ for every $v,v' \in \cV_i$ such that both $A_v \cup B_v \neq \emptyset$ and $A_{v'} \cup B_{v'} \neq \emptyset$. 
	\end{proposition}

%\begin{claim}[Round 0 Claim]\label{cl:round-0}
	%	Let $A , B \subset \{0,1\}^d$, $T$ be a quadtree, and $i \in \{0,\dots, h-1\}$. 
%	Let $\calbE_0$ be the event	that $h(v) \neq h(v')$ for every $v,v' \in \cV_i$ such that both $A_v \cup B_v \neq \emptyset$ and $A_{v'} \cup B_{v'} \neq \emptyset$. %	that the partition $\bV_1, \dots, \bV_{s'}$ of $\cV_i$ satisfies that each set $\bV_j$ contains at most one node $v \in \cV_i$ where $A_v \cup B_v \neq \emptyset$.
%	Then event $\calbE_0$ occurs with probability at least $1 - 1/s$ over the draw of the partition $h$.
%\end{claim}

\begin{proof}
	This simply follows from the fact that $s'$ is at least $8s^3$, and there are at most $2s$ nodes $v \in \cV_{i-1}$ where $A_v \cup B_{v} \neq \emptyset$. Hence, the probability that two non-empty nodes collide in $\bh_{i-1}$ is at most $1/(8s^3)$ (where we use $2$-wise independence), and we may union bound over at most $4s^2$ pairs of non-empty nodes. The same argument can be made that $\bh_i$ perfectly hashes all non-empty nodes in $\cV_i$ with probability $1-1/(2s)$. Conditioned on this, there is a bijection between non-zero terms in $\cbI_i$ and $\cbI_i'$, where terms mapped to each other are equal. 
\end{proof}

Proposition \ref{prop:unireduce} demonstrates that it will be sufficient to estimate $\cbI_i'$. Thus, we condition on the success of this universe reduction step now. Since conditioned on this step the non-zero edges $(\cV_{i-1},\cV_{i})$ are in bijective correspondence with the non-zero edges of $(\cV_{i-1}',\cV_{i}')$, and moreover since under this equivelance the points contained in $A_v,B_v$ and the centers $\bc_v$ are equivalant, in the following we will abuse notation and drop the prime notation in $\cbI_i',\cV_i',\cV_{i-1}'$, and simply write $\cbI_i,\cV_i,\cV_{i-1}$, with the understanding that the universe reduction step has already been carried out.


\subsubsection{Sketching Tools.} 
We will need the following two ingredients for the protocol and the proof.
 


\subsubsection{Description and Analysis of Two-Round Sketch}

We give a description of the two-round protocol, and the precise formulation is given in Figure~\ref{fig:2-round}. As we explain the protocol we specify some claims, which are then combined to prove Theorem~\ref{thm:two-pass}.

\paragraph{Round $0$.} We begin by mapping the vector $f_{A,B} \in \R^{2^{d+1}}$ to a vector $f^i \in \R^{|\cV_i| \times \{A,B\}}$ indexed by vertices $v \in \cV_i$ and $\{A ,B\}$ via
\[	f^i_{v,A}= \sum_{\substack{\vec{x}\in \{0,1\}^d\\ v_i(\vec{x}) = v } } (f_{A,B})_x = |A_v|	\quad \text{and} \quad  	f^i_{v,B}= \sum_{\substack{\vec{x}\in \{0,1\}^d\\ v_i(\vec{x}) = v } } (f_{A,B})_{x + 2^d} = |B_v| \] 
where $\vec{x} \in \{0,1\}^d$ and $x \in [2^d]$ is the index in $[2^d]$ that $\vec{x}$ encodes. In other words, $f^{i}_{v, A}$ and $f^i_{v, B}$ hold the frequency counts of points in $A$ and $B$, respectively, at vertex $v \in \cV_i$, which is a linear mapping of the input $f_{A,B}$. Recall we assume the universe reduction has already been performed, so $|\cV_i| = O(s^6)$. At this point, we initialize sketches to perform $\ell_1$-sampling and $\ell_1$-sketching.

\paragraph{Round 1.} At the end of round 1, the estimate $\hat{\bbeta} \in \R$ is the result of an $\ell_1$-sketch on the vector $F^i$. In other words, we will have that $\hat{\bbeta}$ is a constant factor approximation to $\| F^i\|_1$. Furthermore, the indices $v_1, \dots, v_k \in \calV_i \cup \{ \bot \}$ represent $\ell_1$-samples from $F^i$; while the $\ell_1$-sample does not fail (i.e., $v_t \neq \bot$), the sample $v_t \in \calV_i$ is meant to be distributed proportional to $F^i_{v_t}$. Specifically, we have the following two claims:
\begin{claim}[Round 1 Claim A]\label{cl:round-1-A}
%Consider a fixed partition $(\bV_1, \dots, \bV_{s'})$ of $\cV_i$, and suppose $\calbE_0$ occurs. 
Let $\calbE_1$ be the event, defined over the randomness of the sample $\bC \sim \calS_k^1((s')^3, O(1))$ in Line~\ref{ln:sample-ell-1-sk} of Round 0 that in Line~\ref{ln:eval-1} of Round 1,
\begin{align} 
\sum_{v \in \cV_i} \big| |A_v| - |B_v| \big| \leq \hat{\bbeta} \leq 2  \sum_{v \in \cV_i} \big| |A_v| - |B_v| \big|.  \label{eq:bbeta-bound}
\end{align}
Then, $\calbE_1$ occurs with probability at least $0.99$.
\end{claim}

\begin{proof}
This is a consequence of Theorem~\ref{thm:ell-1-sketch} with $m = (s')^2$, $\delta =.01$, applied to the vector $F^i$ which has $\ell_1$ norm  $\|F^i\|_1 =  \sum_{v \in \cV_i} ||A_v| - |B_v||$%Assuming $\calbE_0$ occurs, we have
%\begin{align*}
%\| \bz^{(A)} - \bz^{(B)} \|_1 &= \sum_{j \in [s']} \left| \sum_{v \in \bV_j} \left(|A_v| - |B_v| \right) \right| = \sum_{v \in \cV_i} \big| |A_v| - |B_v| \big|,
%\end{align*}
%and hence $\hat{\bbeta} = \Alg_{\ell_1\text{-sk}}(\bC (\bz^{(A)}- \bz^{(B)}))$, and we apply Theorem~\ref{thm:ell-1-sketch} with $m = s'$, $\delta = 0.01$, and $x = \bz^{(A)} - \bz^{(B)}$.
\end{proof}

\begin{claim}[Round 1 Claim B]\label{cl:round-1-B}
%Consider a fixed partition $(\bV_1, \dots, \bV_{s'})$ of $\cV_i$, and suppose $\calbE_0$ occurs. 
The random variables $v_1, \dots,v_k$ defined in Line~\ref{ln:eval-1} are independent and identically distributed. We have that $v_t = \bot$ with probability at most $1/3$ for each $t$. Otherwise, for any $v \in \cV_i$ we have
\begin{align*}
\left| \Prx\left[ v_t = v\right] - 
\dfrac{\big| |A_v| - |B_v| \big|}{\sum_{v' \in \cV_i} \big| |A_{v'}| - |B_{v'}|\big|} \right| \leq \frac{1}{s^{10}}. 
\end{align*}
\end{claim}

\begin{proof}
We first note that independence follows from the fact that the random variables $v_1, \dots, v_k$ depend on the independent samples $(\bS_t, \Alg_{\bS_t}^{1}) \sim \calS_{a}^1((s')^2, O(\log^2 s))$ for $t \in [k]$ of Line~\ref{ln:sample-ell-1-sa} of Round 0. The distributional bound then follows from Theorem~\ref{thm:ell-1-sa} with $c=10$, applied to the input vector $F^i$.

%for any $t \in [k]$, we apply Theorem~\ref{thm:ell-1-sa} with $m = s'$ to the vector $\bz^{(A)} - \bz^{(B)}$ and $j \in [s']$ with $c = 10$ with the sample $(\bS_t, \Alg_{\bS_t}^{(\ell_1\text{-sa})}) \sim \calD_{\ell_1\text{-sa}}(s', O(\log^2 s))$.
\end{proof}

\paragraph{Round 2.} The second round is meant to communicate, for each $t \in [k]$, the information necessary to estimate $\bq_{\pi(v_t), v_t}$. In order to do this, the players must jointly approximate $\| c_{\pi(v_t)} - c_{v_t}\|_1$. For each $t \in [k]$, $n_t$ is the number of points in $A$ and $B$ which lie in $\pi(v_t)$, and notice that, once both players know $v_t$, $n_t$ can be computed exactly by communicating $|A_{\pi(v_t)}|$ and $|B_{\pi(v_t)}|$ with $O(\log s)$ bits. The centers of mass, $c_{v_t}$ and $c_{\pi(v_t)}$ are given by the vectors
\begin{align*} 
c_{v_t} &= \frac{1}{f^i_{v_t, A} + f^i_{v_t,B}}\sum_{\substack{\vec{x} \in \{0,1\}^d \\ v_{i}(\vec{x}) = v_t}} \vec{x} \left((f_{A,B})_{x} + (f_{A,B})_{x + 2^d} \right) \\
 c_{\pi(v_t)} &= \frac{1}{n_t} \sum_{\substack{\vec{x} \in \{0,1\}^d \\ v_{i-1}(\vec{x}) = \pi(v_t) }} \vec{x} \left( (f_{A,B})_{x} + (f_{A,B})_{x + 2^d} \right).
 \end{align*}
 Therefore, $\bchi_t^i$ is an $\ell_1$-sketch of $(f^i_{v_t, A} + f^i_{v_T, B}) c_{v_t}$ and $\bchi_t^{i-1}$ an $\ell_1$-sketch of $n_t c_{\pi(v_t)}$ such that $\|c_{\pi(v_t)} - c_{v_t}\|_1$ can be approximated, and $\hat{\bq}_t$ becomes an approximation of $\bq_{\pi(v_t), v_t}$. This last point is captured by the following claim.
 
 \begin{claim}[Round 2 Claim]\label{cl:round-2}
%Consider a fixed partition $(\bV_1, \dots, \bV_{s'})$ of $\cV_i$, and suppose $\calbE_0$ occurs. 
Let $v_t \in \cV_i$ be any sample returned by Line \ref{ln:eval-1} in Round 1, and suppose $v_t \neq \bot$.
%Let $j \in [s']$ such that $\bV_j$ contains a unique node $v^*$ where $A_{v^*} \cup B_{v^*} \neq \emptyset$, and $u^*$ be its parent. For any $t \in [k]$, suppose $\bj_t = j$ is a realization of the random variable defined in Line~\ref{ln:eval-1} of Round 1.
 Let $\calbE_{2, t}$ be the event, defined over the randomness of the sample $\bC_t \sim \calS_{k}^1(d, O(\log\log s))$ in Line~\ref{ln:sample-ell-1-sk} of Round 0 that in Line~\ref{ln:eval-2} of Round 2,
\begin{align*}
\left\| \bc_{v^*} - \bc_{u^*}  \right\|_1 \leq \Alg^{1}\left( \dfrac{\bchi_t^{i-1} }{\boldn_t} - \dfrac{\bchi_t^{i}}{f^i_{v_t,a} + f^i_{v_t,b}} \right)\leq 2\left\| \bc_{v^*} - \bc_{u^*}  \right\|_1.
\end{align*}
Then, $\calbE_{2, t}$ occurs with probability at least $1 - 1/(100 k)$.
\end{claim}

\begin{proof}
We apply Theorem~\ref{thm:ell-1-sketch} with $m = d$, $t = O(\log\log s)$, and notice by definition
\[\dfrac{\bchi_t^{i-1} }{n_t} = \frac{\sum_{\substack{\vec{x} \in \{0,1\}^d \\ v_{i-1}(x) = \pi(v_t)}} (\bC_t \vec{x}) \cdot( (f_{A,B})_x + (f_{A,B})_{x+ 2^d}) }{|A_{\pi(v_t)}| + |B_{\pi(v_t)}|} =\frac{\sum_{x \in A_{\pi(v_t)}  \cup B_{\pi(v_t)}} \bC_t x }{|A_{\pi(v_t)}| + |B_{\pi(v_t)}|} = \CC_t \cdot c_{\pi(v_t)} \]
similarly 
\[\dfrac{\bchi_t^{i} }{f_{v_t,a}^i + f^i_{v_t,b}} = \frac{\sum_{\substack{\vec{x} \in \{0,1\}^d \\ v_{i}(x) = v_t}} (\bC_t \vec{x}) \cdot( (f_{A,B})_x + (f_{A,B})_{x+ 2^d}) }{|A_{v_t}| + |B_{v_t}|} =\frac{\sum_{x \in A_{v_t}  \cup B_{v_t}} \bC_t x }{|A_{v_t}| + |B_{v_t}|} = \CC_t \cdot c_{v_t} \]
% \qquad 	\bchi_t^{i-1} &\eqdef \sum_{\substack{\vec{x} \in \{0,1\}^d \\ v_{i-1}(x) = \pi(v_t)}} (\bC_t \vec{x}) \cdot( f^i_x + f^i_{x+ 2^d})\\
thus, by linearity
\[	 \dfrac{\bchi_t^{i-1} }{n_t} - \dfrac{\bchi_t^{i}}{f^i_{v_t,a} + f^i_{v_t,b}} = \bC_t (c_{v_t} - c_{\pi(v_t)}) 	\]
where $ \bC_t \sim \calS_{k}^1(d, O(\log\log s))$, and noting that $k = O(\log s)$ so the failure probability of Theorem~\ref{thm:ell-1-sketch}  is $1/\poly(k)$.
 %and vector $x \in \R^d$ given by
%\begin{align*}
 %x &= \frac{1}{\boldn_t^{(v, A)} + \boldn_t^{(v, B)}}\sum_{v \in \bV_j} \sum_{\substack{y \in A \cup B \\ v_{i, T}(y) = v}} y - \frac{1}{\boldn_t^{(u, A)} + \boldn_t^{(u, B)}}\sum_{v \in \bV_j} \sum_{\substack{y \in A \cup B \\ v_{i-1, T}(x) = \pi(v)}} y \\
 %   &= \frac{1}{|A_{v^*} \cup B_{v^*}|}\sum_{y \in A_{v^*} \cup B_{v^*}} y - \frac{1}{|A_{u^*} \cup B_{u^*}|} \sum_{y \in A_{u^*} \cup B_{u^*}} y = \bc_{v^*} - \bc_{u^*} ,
 %\end{align*}
 %where in the second equality, we used the fact that $v^*$ is the unique node in $\bV_{j}$ with non-empty $A_{v^*} \cup B_{v^*}$, and $u^*$ is its parent in order to conclude $\boldn_t^{(v, A)} = |A_{v^*}|$, $\boldn_t^{(v, B)} = |B_{v^*}|$, $\boldn_{t}^{(u, A)} = |A_{u^*}|$ and $\boldn_t^{(u, B)} = |B_{u^*}|$. We note that in Line~\ref{ln:vectors-to-send} of Round 2,
 %\begin{align*}
 %\bchi_t^{(v, A)} + \bchi_{t}^{(v, B)} &= \bC_t \left( \sum_{v \in \bV_j} \sum_{\substack{y \in A \\ v_{i, T}(y) = v}} y + \sum_{v \in \bV_j} \sum_{\substack{y \in B \\ v_{i, T}(y) = v}} y \right) \\
 %\bchi_t^{(u, A)} + \bchi_{t}^{(u, B)} &= \bC_t \left(\sum_{v \in \bV_j} \sum_{\substack{y \in A \\ v_{i-1, T}(y) = \pi(v)}} y + \sum_{v \in \bV_j} \sum_{\substack{y \in B \\ v_{i-1, T}(y) = \pi(v)}} y \right), 
 %\end{align*}
%which means we may apply Theorem~\ref{thm:ell-1-sketch}, and the final bound follows from the fact $k = O(\log s)$.
\end{proof}

\begin{figure}[H]
	\begin{framed}
		\noindent Two-round Sketch $\hspace{0.04cm} (f_{A,B}, T, i)$
		
		\begin{flushleft}
			\noindent {\bf Input:} Vector $f_{A,B} \in \R^{2^{d+1}}$ encoding two multi-sets $A, B \subset \{0,1\}^d$, a compressed quadtree $T$, and index $i\in \{0 ,\dots, h-1\}$.
			
			\noindent {\bf Output:} A real number $\hat{\calbI}_i$. % or ${\reject}$.
			
			\begin{itemize}
				\item Round 0: Perform the universe reduction step (Proposition \ref{prop:unireduce}) so that $|\cV_{i-1}| = s', |\cV_{i}| = (s')^2$, where $s' = O(s^3)$. Set $k = O(\log^2 s)$.
				\begin{enumerate}
				\item Define the linear functions $f^i \in \R^{|\cV_i| \times \{A,B\}}$ and $F^i \in \R^{|\cV_i|}$ of $f_{A,B}$ via
		
			\[	f^i_{v,A}= \sum_{\substack{\vec{x}\in \{0,1\}^d\\ v_i(\vec{x}) = v } } (f_{A,B})_x = |A_v|	\quad \text{and} \quad  	f^i_{v,B}= \sum_{\substack{\vec{x}\in \{0,1\}^d\\ v_i(\vec{x}) = v } } (f_{A,B})_{x + 2^d} = |B_v| \] 
			\[	F^i_v = f^i_{v,A} - f^i_{v,B}	= |A_v| - |B_v|\]
			%	\item Sample random hash function $h: \cV_i \to [s']$.
				\item\label{ln:sample-ell-1-sa} For each $t \in [k]$, initialize linear sketch $(\bS_t, \Alg_{\bS_t}^{1}) \sim \calS_a^1((s')^2,O(\log^2 s))$.
				\item\label{ln:sample-ell-1-sk} For each $t \in [k]$, initialize linear sketch $\bC_t \sim \calS_{k}^1(d, O(\log \log s))$, and initialize $\bC \sim \calS_{k}^1((s')^2, O(1))$.
				\end{enumerate}
				\item Round 1: 
				\begin{enumerate}
					
					\item Construct the linear sketch $\bbeta \eqdef \bC F^i$, and for each $t \in [k]$, construct the linear sketches $\balpha_t \eqdef \bS_{t} F^i$.
					\item\label{ln:eval-1} Generate $k$ samples $v_1, \dots,v_k \in \cV_i \cup \{\bot\}$ obtained from 
					\[ v_t \eqdef \Alg_{\bS_t}^{1}(\balpha_t ), \qquad\text{and let}\qquad \hat{\bbeta} \eqdef \Alg^{1}(\bbeta).  \]
				\end{enumerate}
				\item Round 2: Let $L \subset [k]$ be the set of indices such that $v_t \neq \bot$. For each $t \in L$:  
		
			%	compute the quantities 
			%	\begin{align*}
			%	\boldn_t^{(v,A)} &\eqdef  f_x^i \qquad \boldn_t^{(u, A)} \eqdef \sum_{\substack{x \in \{0,1\}^d \\ \exists v \in \cV_i\text{ s.t. } h(v)  = j_t \\ \text{and } \pi(v) = v_{i-1}(x)}} f_x^i \ \\
			%	\boldn_t^{(v,B)} &\eqdef \sum_{\substack{x \in \{0,1\}^d \\ h(v_i(x)) = j_t }} f_{x+2^d}^i  \qquad \boldn_t^{(u, B)} \eqdef \sum_{\substack{x \in \{0,1\}^d \\ \exists v \in \cV_i\text{ s.t. } h(v)  = j_t \\ \text{and } \pi(v) = v_{i-1}(x)}} f_{x+2^d}^i
			%	\end{align*}
				\begin{enumerate}
							\item Compute the value $n_t \eqdef   \sum_{\substack{v \in \cV_i\\ \pi(v) = \pi(v_t) }} f^i_{v,A} + f^i_{v,B} = |A_{\pi(v_t)}| + |B_{\pi(v_t)}|$. 
							
				\item\label{ln:vectors-to-send} Compute the vectors
				\begin{align*}
				\hspace{-1.5cm}\bchi_t^{i} &\eqdef \sum_{\substack{\vec{x} \in \{0,1\}^d \\ v_{i}(\vec{x}) = v_t}} (\bC_t \vec{x}) \cdot( (f_{A,B})_x + (f_{A,B})_{x+ 2^d}) , \qquad 	\bchi_t^{i-1} &\eqdef \sum_{\substack{\vec{x} \in \{0,1\}^d \\ v_{i-1}(\vec{x}) = \pi(v_t)}} (\bC_t \vec{x}) \cdot( (f_{A,B})_x + (f_{A,B})_{x+ 2^d}).
				\end{align*}
				\item \label{ln:eval-2} Let
				 \[ \hat{\bq}_t \eqdef \max \left\{ \min\left\{ \Alg^{1}\left( \dfrac{\bchi_t^{i-1} }{n_t} - \dfrac{\bchi_t^{i}}{f^i_{v_t,A} + f^i_{v_t,B}} \right), \frac{30d \log s}{2^i} \right\}, \frac{d}{2^i} \right\} ,\]
				 if all $\boldn_t$ and $f^i_{v_t,A} + f^i_{v_t,B}$ are non-zero. Output
				\begin{align*}
					\hat{\cbI}_i \eqdef \hat{\bbeta} \cdot \frac{1}{|L|} \sum_{t \in L} \hat{\bq}_t.
				\end{align*}
				\end{enumerate}
			\end{itemize}
		\end{flushleft}\vskip -0.14in
	\end{framed}\vspace{-0.2cm}
	\caption{The Two-round Protocol.}\label{fig:2-round}
\end{figure}

\begin{proofof}{Theorem~\ref{thm:two-pass}}
As mentioned in the paragraph subsequent to stating Theorem~\ref{thm:two-pass}, we show that for any compressed quadtree $T$ and any $i \in \{0, \dots, h-1\}$, with probability at least $3/4$ over the execution of the sketching algorithm, the output $\hat{\cbI}_i$ satisfies $\cbI_i/8 \leq \hat{\cbI}_i \leq 8 \cbI_i$. Repeating the protocol for $O(\log \log d)$ iterations and outputting the median (in order to decrease the error probability), and repeating it for all $i \in \{0, \dots, h-1\}$ obtains the desired theorem.

For the rest of the proof, consider a fixed $i \in \{0, \dots, h-1\}$ and $T$. % By Claim~\ref{cl:round-0}, consider the case $\calbE_0$ occurs (which occurs with probability $1 - 1/s$, so that we may ignore cases where $\calbE_0$ does not occur).
 We consider the distribution $\nu$ supported on $\cV_i$ where
\begin{align*}
\Prx_{\bv \sim \nu}\left[\bv = v^*\right] \propto \big|  |A_{v^*}| - |B_{v^*}| \big|, \qquad\text{and}\qquad Z \eqdef \sum_{v \in \cV_i} \big|  |A_v| - |B_v|\big|
\end{align*}
is the normalizing constant. %Notice that whenever $\calbE_0$ occurs, each $\bV_j$ contains at most one node $v$ where $A_{v} \cup B_{v}$ is non-empty. 
%For each $j \in [s']$, let $v_j \in \cV_i$ be the unique node in $\bV_j$ where $A_v \cup B_{v} \neq \emptyset$ if one exists, and an arbitrary node in $\bV_j$ otherwise (in particular, if $A_v \cup B_v =\emptyset$ for all $v \in V_j$, then $\Pr_{\bj \sim \nu}[\bj = j] = 0$). 
%Then, we have 
%\[ \Prx_{\bj \sim \nu}\left[ \bj = j^*\right] \propto \big| |A_{v_j}| - |B_{v_j}| \big|, \qquad\text{and}\qquad Z = \sum_{v \in \cV_i} \big| |A_{v}| - |B_v| \big|. \]
We have
\begin{align*}
\calbI_i = Z \cdot \Ex_{\bv \sim \nu}\left[ \bq_{\bv, \pi(\bv)}\right] \geq Z \cdot \frac{d}{2^i}.
\end{align*}
To complete the proof, we show the following:
\begin{enumerate}
\item\label{en:first-to-show} The random variable $\hat{\bbeta}$ satisfies $Z \leq \hat{\bbeta} \leq 2 Z$, with probability at least $0.99$ over the randomness in $\bC \sim \calS_k^1((s')^3, O(1))$. This follows immediately from Claim~\ref{cl:round-1-A}.
\item\label{en:second-to-show} For every $t \in L$, consider the sample $v_t \in \cV_i$ in Line~\ref{ln:eval-1} of Round 1. Then, with probability at least $1 - 1/(100k)$ over the draw of $\bC_t \sim \calS_k^1(d, O(\log\log s))$,
 \[ \frac{d}{2^i} \leq \bq_{v_j, u_j} \leq \hat{\bq}_t \leq 2 \bq_{v_j, u_j} \leq \frac{60 d \log s}{2^i},\]
which follows from Claim~\ref{cl:round-2}.
\item We have $|L| > k/2$ with probability $1-1/s$. This follows from a Chernoff bound on the number of $v_t$ such that $v_t = \bot$. 

\item\label{en:js-ind-and-vu} The random variables $v_i$ for $i \in [L]$ in Line~\ref{ln:eval-1} are independent and identically distributed, depending on the draw of $(\bS_t, \Alg_{\bS_t}^{(\ell_1\text{-sa})}) \sim \calS_a^1((s')^2, O(\log^2 s))$. Specifically, they are drawn from a distribution $\calD'$ over $\cV_i$, such that we have $\dtv(\calD', \nu) \leq 1/s$. 
% For each $t \in [k]$, $\bV_{\bj_t}$ contains a unique node $v$ where $A_{v} \cup B_v \neq \emptyset$ with probability $1-1/s^7$, which implies $\boldn_t^{(v, A)} + \boldn_t^{(v, B)}$ and $\boldn_t^{(u,A)} + \boldn_t^{(u,B)}$ are both non-zero. Letting $\calD'$ denote the distribution from which $\bj_t$ is sampled conditioned on this event, we have $\dtv(\calD', \nu) \leq 1/s$. 
This follows from Claim~\ref{cl:round-1-B}.
\end{enumerate}
From $1$ and $4$ above, we have that with probability at least $0.99$, 
\[  \cbI_i / 2 \leq \cbI_i - O\left( \frac{Z \cdot d \log s}{s2^i}\right) \leq \Ex_{\bv  \sim \calD'}\left[ \hat{\bbeta} \cdot \bq_{\bv, \pi(\bv)}  \right]  \leq  \cbI_i + O\left( \frac{Z \cdot d\log s}{s 2^i}\right) \leq 2 \cbI_i\]
and by 2, with probability $0.99 \cdot 0.99$ over the draws of $\bC \sim \calS_k^1((s')^2, O(1))$ and all $\bC_1, \dots ,\bC_k \sim \calS_k^1(d, O(\log \log s))$,
\[ \frac{1}{4} \cdot \cbI_i \leq \Ex_{\bv \sim \calD'}\left[ \hat{\bbeta} \cdot \hat{\bq}_{t} \right] \leq 4 \cbI_i \]
%Finally, note that since the draws of $\bj_1, \dots, \bj_k$ are independent, with probability at least $1 - k / s^7$, all draws of $\bj_t$ are distributed according to $\calD'$. 
Thus, the output $\hat{\bq}$ of the sketching algorithm has expectation between $\calbI_i/4$ and $4 \calbI_i$, and by the boundedness of $\hat{\bq}_t$ and independence across $t \in [k]$,
\[ \Var\left[\frac{\hat{\bbeta}}{k} \sum_{t=1}^k \hat{\bq}_t \right] = O\left( \frac{Z^2 d^2 \log^2 s}{k \cdot 2^{2i}}\right),\]
which is less than $c\cbI_i^2$ for arbitrarily small constant $c > 0$, given large enough $k = O(\log^2 s)$. As a result, we apply Chebyshev's inequality to conclude that the output $\hat{\bq}$ is between $\cbI_i / 8$ and $8\cbI_i$ with probability at least $0.99\cdot 0.99 \cdot 0.99 > 3/4$ as needed, and we conclude the theorem.
\end{proofof}
